Zero-Shot Subject-Centric Generation for Creative Application Using Entropy Fusion

Generative models are widely used in visual content creation. However, current text-to-image models often face challenges in practical applications-such as textile pattern design and meme generation-due to the presence of unwanted elements that are difficult to separate with existing methods. Meanwhile, subject-reference generation has emerged as a key research trend, highlighting the need for techniques that can produce clean, high-quality subject images while effectively removing extraneous components. To address this challenge, we introduce a framework for reliable subject-centric image generation. In this work, we propose an entropy-based feature-weighted fusion method to merge the informative cross-attention features obtained from each sampling step of the pretrained text-to-image model FLUX, enabling a precise mask prediction and subject-centric generation. Additionally, we have developed an agent framework based on Large Language Models (LLMs) that translates users' casual inputs into more descriptive prompts, leading to highly detailed image generation. Simultaneously, the agents extract primary elements of prompts to guide the entropy-based feature fusion, ensuring focused primary element generation without extraneous components. Experimental results and user studies demonstrate our methods generates high-quality subject-centric images, outperform existing methods or other possible pipelines, highlighting the effectiveness of our approach.

==> matting.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{matting_1.pdf}
    \caption{Comparison between the proposed method and 2 matting methods. The \textcolor{red}{red arrows} indicate the area where the matting method's predictions are incorrect.}
    \label{fig:figurematting}
    \centering
\end{figure}


==> tab_temp1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!t]
\scriptsize
   \centering
   \caption{The details of 14 open-sourced fundus datasets used in our RVS benchmark. Based on different experimental purposes, they were classified into 3 label sources, 1 unlabeled set, and 10 datasets for DG evaluation. The official data partitioning (train/test) was adopted for the label sources, whereas the evaluation datasets were not partitioned as they were tested as a whole. $\#$ represents the number of images.}
   \label{tab:datasets}
  	\resizebox{\textwidth}{!}{%调整大小
\begin{tabular}{c | c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} | c@{\hspace{4pt}} | c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}} c@{\hspace{4pt}}}\hline
 & \multicolumn{3}{c|}{Labeled Sources} & Unlabeled & \multicolumn{10}{c}{Domain Generalization Evaluation Benchmark} \\ 
\hline
% Dataset & HRF~\cite{budai2013robust} & STARE~\cite{hoover2000locating} & CHASEDB1~\cite{owen2009measuring} & DRIVE~\cite{staal2004ridge} & ARIA~\cite{farnell2008enhancement} & IOSTAR~\cite{zhang2016robust} & ORVS~\cite{sarhan2021transfer} & DR-HAGIS~\cite{holm2017dr} & AFIO~\cite{akbar2017avrdb} & FIVES~\cite{jin2022fives} & LES-AV~\cite{orlando2018towards} & RETA~\cite{lyu2022reta} & TREND~\cite{popovic2021trend}\\
% \hline
Dataset & HRF & STARE & CHASEDB1 & EyePACS & DRIVE & ARIA & IOSTAR & ORVS & DR-HAGIS & AFIO & FIVES & LES-AV & RETA & TREND\\
\hline
% Diversity & Low & Low & Low & Low & Med. & Low & Low & Low & Low & Med. & Low & Low & Low\\
% \hline
% Quality & High & Low & Med. & High & Med. & High & Low & High & High & Med. & Med. & Med. & Med.\\
% \hline
Disease & True & True & False & True & True & True & False & False & True & True & True & True & True & False\\
% \hline
% Label Quality & High & Low & Medium & High & Medium & Medium & Medium & Medium & High & Medium & Medium & Medium & Medium\\
\hline
Partition $\#$ & 15 / 30 & 10 / 10 & 20 / 8 & 35,126 & 40 & 142 & 30 & 49 & 40 & 99 & 800 & 22 & 54 & 82 \\
\hline
% Test Data & 30 & 10 & 8 & - & - & - & - & - & - & - & - & - & -\\
% \hline
% In Total & 45 & 20 & 28 & 40 & 142 & 30 & 49 & 40 & 99 & 800 & 22 & 54 & 82\\
% \hline
\end{tabular}} % 这里还有一个调整大小的结束括号，即是对表格整体调整大小
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h!t]
% \scriptsize
%    \centering
%    \caption{Open-sourced fundus datasets.}
%    \label{tab:datasets2}
%   	\resizebox{\textwidth}{!}{%调整大小
% \begin{tabular}{c | c | c | c | c | c | c | c}\hline
%  \multicolumn{2}{c|}{Dataset Information} & \multicolumn{3}{|c}{Dataset Characteristic} & \multicolumn{3}{|c}{Data Number}\\ 
% \hline
% Types & Dataset Names & Image Diversity & With Disease & Image Quality & Training Set & Test Set & In Total\\
% \hline

% Unlabeled Datasets & EyePACS & Low & x & x & x & x & x  \\
% \hline
% % \cline{2-8}
% \multirow{3}{*}{Labeled Datasets} & HRF~\cite{budai2013robust} & High & x & x & x & x & x \\
% % \hline
% \cline{2-8}
%  & STARE~\cite{hoover2000locating} & High & x & x & x & x & x \\
% % \hline
% \cline{2-8}

%  & CHASEDB1~\cite{owen2009measuring} & - & x & x & x & x & x\\
%  \hline
% % \cline{2-8}
% \multirow{10}{*}{Datasets for Evaluation} & DRIVE~\cite{staal2004ridge} & True & x & x & x & x & x  \\
% % \hline
% \cline{2-8}
%  & ARIA~\cite{farnell2008enhancement} & - & x & x & x & x & x   \\
% % \hline
% \cline{2-8}

%  & IOSTAR~\cite{zhang2016robust} & - & x & x & x & x & x\\
%  % \hline
% \cline{2-8}
%  & ORVS~\cite{sarhan2021transfer} & True & x & x & x & x & x  \\
% % \hline
% \cline{2-8}
%  & DR-HAGIS~\cite{holm2017dr} & - & x & x & x & x & x  \\
%  \cline{2-8}
%  & AFIO~\cite{akbar2017avrdb} & - & x & x & x & x & x  \\
%  \cline{2-8}
%  & FIVES~\cite{jin2022fives} & - & x & x & x & x & x  \\
%  \cline{2-8}
%  & LES-AV~\cite{orlando2018towards} & - & x & x & x & x & x  \\
%  \cline{2-8}
%  & RETA~\cite{lyu2022reta} & - & x & x & x & x & x  \\
%  \cline{2-8}
%  & TREND~\cite{popovic2021trend} & - & x & x & x & x & x  \\
% \hline

% \end{tabular}}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}
%   \centering
%   \caption{Open-sourced fundus datasets.}
%   \label{tab:datasets3}
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{c | c | c | c | c | c | c | c}\hline
%  \multicolumn{2}{c|}{Dataset Information} & \multicolumn{3}{|c}{Characteristic} & \multicolumn{3}{|c}{Characteristic}\\ 
% \hline
% Types & Datasets & \shortstack{Image\\ Diversity} & \shortstack{With \\Disease} & \shortstack{Image\\ Quality} & \shortstack{Training \\Set} & \shortstack{Test \\Set} & \shortstack{In \\Total}\\
% \hline

% \multirow{3}{*}{\shortstack{Labeled\\Datasets}} & HRF~\cite{budai2013robust} & Low & x & x & x & x & x  \\
% % \hline
% \cline{2-8}
%  & STARE~\cite{hoover2000locating} & High & x & x & x & x & x \\
% % \hline
% \cline{2-8}
%  & CHASEDB1~\cite{owen2009measuring} & High & x & x & x & x & x \\
% \hline

% \multirow{3}{*}{\shortstack{Datasets \\for\\Evaluation}} & HRF~\cite{budai2013robust} & - & x & x & x & x & x\\
%  % \hline
% \cline{2-8}
%  & STARE~\cite{hoover2000locating} & True & x & x & x & x & x  \\
% % \hline
% \cline{2-8}
%  & CHASEDB1~\cite{owen2009measuring} & - & x & x & x & x & x   \\
% \hline

% \multirow{3}{*}{SAM} & HRF~\cite{budai2013robust} & - & x & x & x & x & x\\
%  % \hline
% \cline{2-8}
%  & STARE~\cite{hoover2000locating} & True & x & x & x & x & x  \\
% % \hline
% \cline{2-8}
%  & CHASEDB1~\cite{owen2009measuring} & - & x & x & x & x & x  \\
% \hline

% \multicolumn{2}{c|}{Ours (TransUnet)} & 40 & x & x & x & x & x \\
% \hline
% \end{tabular}}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tab_temp2.tex <==
\begin{table}
  \centering
  \caption{Comparisons SOTAs with/without pseudo labels re-training.}
  \label{tab:initialtraining}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{c | c | c | c | c}\hline
 \multicolumn{2}{c|}{Varying Label Sources Training} & \multicolumn{3}{|c}{Unseen Datasets Evaluation} \\ 
\hline
Methods & Label Sources & Initial Stage & Full Stage & Difference\\
\hline

\multirow{3}{*}{ST++} & HRF~\cite{budai2013robust} & Low & x & x  \\
% \hline
\cline{2-5}
 & STARE~\cite{hoover2000locating} & High & x  & x \\
% \hline
\cline{2-5}
 & CHASEDB1~\cite{owen2009measuring} & High & x  & x  \\
\hline

\multirow{3}{*}{UniMatch} & HRF~\cite{budai2013robust} & - & x & x \\
 % \hline
\cline{2-5}
 & STARE~\cite{hoover2000locating} & True & x  & x \\
% \hline
\cline{2-5}
 & CHASEDB1~\cite{owen2009measuring} & - & x  & x  \\
\hline

\multirow{3}{*}{Ours} & HRF~\cite{budai2013robust} & - & x & x\\
 % \hline
\cline{2-5}
 & STARE~\cite{hoover2000locating} & True & x  & x  \\
% \hline
\cline{2-5}
 & CHASEDB1~\cite{owen2009measuring} & - & x  & x  \\
\hline

\multicolumn{2}{c|}{Ours (TransUnet)} & 40 & x & x \\
\hline
\end{tabular}}
\end{table}
